Efficient and Generic Algorithms for Quantitative Attack Tree Analysis

Numerous analysis methods for quantitative attack tree analysis have been proposed. These algorithms compute relevant security metrics, i.e. performance indicators that quantify how good the security of a system is; typical metrics being the most likely attack, the cheapest, or the most damaging one. However, existing methods are only geared towards specific metrics or do not work on general attack trees. This paper classifies attack trees in two dimensions: proper trees vs. directed acyclic graphs (i.e. with shared subtrees); and static vs. dynamic gates. For three out of these four classes, we propose novel algorithms that work over a generic attribute domain, encompassing a large number of concrete security metrics defined on the attack tree semantics; dynamic attack trees with directed acyclic graph structure are left as an open problem. We also analyse the computational complexity of our methods.

==> algo_is_well_formed.tex <==
% !TEX root =  main.tex

\begin{algorithm}
	\def\edges{\ensuremath{\mathit{edges}}}
	\KwIn{Dynamic attack tree $\T=(\ATnodes,\typOp,\chOp)$.}
	\KwOut{Whether \T is a well-formed \DAT.}
	%\BlankLine
	\edges\ := $\emptyset$\\
	\ForEach{$\SAND(v_1,\ldots,v_{n+1})\in\ATnodes$}{%
		\For{$i=1$ \KwTo $n$}{%
			\edges\ := $\edges \cup \big(\desc(v_i)\times\desc(v_{i+1})\big)$
		}
	}
	\Return{$\nexists~\text{directed cycle in}~\ograph{}=(\BAS,\edges)$}
	\caption{$\iswellformed(\T)$}
	\label{alg:is_well_formed}
\end{algorithm}


==> algo_metric_SAT.tex <==
% !TEX root =  main.tex

\begin{algorithm}
	\DontPrintSemicolon
	\KwIn{Static attack tree $\T=(\ATnodes,\typOp,\chOp)$,\newline
	      attribute domain $\domain=(\Vdom,\operOR,\operAND)$,\newline
	      attribution $\attrOp$.}
	\KwOut{Metric value $\metr{\T}\in\Vdom$.}
	\BlankLine
	\ssem{\T} := $\mathtt{compute\_semantics}(\T)$\\
	\Return{$\bigoperOR_{\attack\in\ssem{\T}}\bigoperAND_{a\in\attack}\attr{a}$}
	\tcp*{two nested loops}
	%
%	% Fully expanded version:
%	\def\arr{\ensuremath{\mathtt{arr}}}
%	\ssem{\T} := $\mathtt{compute\_semantics}(\T)$\\
%	$n$ := number of attacks in \ssem{\T}; $i$ := $0$\\
%	\arr\ := empty array of lenght $n$\\
%	\For (\tcp*[f]{\metr{\T}}) {$\attack\in\ssem{\T}$}{%
%		$a$ := extract \BAS from \attack; $\arr[i]$ := \attr{a}\\
%		\For (\tcp*[f]{\metrA{\attack}}) {$a\in\attack$}{%
%			$\arr[i]$ := $\arr[i] \operAND \attr{a}$
%		}
%		$i$ := $i+1$
%	}
%	\For (\tcp*[f]{\metr{\T}}) {$\attack\in\ssem{\T}$}{%
%		$\arr[i]$ := $\bigoperAND_{a\in\attack} \attr{a}$ ; $i$ := $i+1$
%	}
%	\Return{$\bigoperOR_{i=0}^n \arr[i]$}
	%
	\caption{$\mathtt{metric}$ for an arbitrary \SAT \T}
	\label{alg:metric_SAT}
\end{algorithm}


==> table_AT_classes.tex <==
% !TEX root =  main.tex

\begin{table}[ht]
  \vspace{2.5ex}
  \centering
  %
  \begin{tabular}[t]{m{.45\linewidth}}
	\toprule
	\multicolumn{1}{c}{\scshape\bfseries structure}
	\\\midrule
	\textbf{Tree}: every node has one parent, except the root which has none.
	\\\midrule
	\textbf{\DAG}: at least one node has two or more parents.
	\\\bottomrule
  \end{tabular}
  ~
  \begin{tabular}[t]{@{~}m{.19\linewidth}@{\,}|@{~\,}m{.19\linewidth}@{\;}}
	\toprule
	\multicolumn{2}{c}{\scshape\bfseries components}
	\\\midrule
	\vspace{3ex}\hspace{.3em}\parbox[b][6ex]{.9\linewidth}{\raggedright%
	\textbf{Static}:\\ there is no \SAND gate.}
	&
	\vspace{3ex}\hspace{.3em}\parbox[b][6ex]{.9\linewidth}{\raggedright%
	\textbf{Dynamic}:\\ at least one \SAND gate.}
	\\[5.3ex]\bottomrule
  \end{tabular}

  \medskip
  \caption{Classification of \ATs by structure and components}
  \label{tab:AT_classes}
  \vspace{-2.5ex}
\end{table}

